Extended Corona Models of X-ray Reverberation in the AGN 1H~0707-495 and IRAS 13224-3809

We fit a new vertically extended corona model to previously measured reverberation time lags observed by \emph{XMM-Newton} in two extremely variable Narrow Line Seyfert 1 Active Galactic Nuclei (AGN), 1H~0707-495 and IRAS~13224-3809, in a variety of similarly observed flux groups and explore the model in all observations over a 16 year period. The model employs two X-ray sources located along the black hole rotational axis at height, $h_1$ and $h_2$ respectively. These sources have their associated photon indices $\Gamma_1$ and $\Gamma_2$ which respond to fluctuations in the disc with a maximum response duration of $t_\text{max}$ and a propagation delay between the response of the two of $t_\text{shift}$. We find that for 1H 0707-495, $h_2$ is significantly correlated with $\Gamma_1$ and anti-correlated with ionisation $\xi$. Whilst the 1H 0707-495 corona extends upwards, the emission appears softer and the disc is less ionised. We find similarities in IRAS 13224-3809, but significant anti-correlation between $\Gamma_2$ and both $t_\text{max}$ and $t_\text{shift}$. This suggests that when the IRAS 13224-3809 corona becomes softer while extending vertically upwards, the overall corona response occurs faster. This may also suggest that the inner disc also becomes more active. In addition, $\Gamma_1$ and $\Gamma_2$ are extreme, relatively less variable, but more separate in IRAS 13224-3809 than in 1H 0707-495. This suggests that the IRAS 13224-3809 corona may be more patchy in the sense that it has two more clear distinct spectral zones of $\Gamma_1$ and $\Gamma_2$ (possibly relating to two distinct zones of coronal temperature) when compared to 1H 0707-495.

==> removed.tex <==
\subsection{Extended Corona Modelling}

The Extended Corona model was also developed using the Interactive Spectral Interpretation System (ISIS) Version 1.6.2-27. The full results of model parameters of 1~H0707-495 are presented in Table~\ref{1H_ecm_results}, outlining all individual observations including the combinations of various epochs explored. Generally, much better fits were obtained using single observations than combining the observations into spectral groupings. Although spectral combinations are useful for obtaining snapshots of the various epochs, the true variability is best revealed by examining each observation in turn however this is time consuming and computationally expensive. We independently examined the posterior distribution for the mass using only the single observation best fits. For this inspection we use the MCMC Hammer \citep{2013PASP..125..306F} and initiate 100 walkers with 100 burn-in steps and run the chain with 100,000 iterations to obtain a mass log$M~M_{\odot} = 6.18 \pm 0.04$, where the errors are calculated at the 90\% confidence limit. The posterior density is shown in Figure~\ref{fig:1h_mass_distribution}. This value is slightly lower than that reported in the literature \citep[e.g.][]{2010MNRAS.401.2419Z, Zhou_2004} although uncertainties in the estimations have been acknowledged.

\begin{figure}
    \centering
    \includegraphics[width=9.5cm]{images/1H0707-mass-density-histogram.pdf}
    \caption{The posterior density for all individual observations of 1H0707-495 showing the mean mass $\mu$ = 6.18 (solid black line) and $\sigma$ = 0.17 (blue region). The Median value was 6.19. }
    \label{fig:1h_mass_distribution}
\end{figure} 


\begin{figure}
    \centering
    % PATH = /home/steff075/phd_ecm/1h0707/1H0707-lag-results-All-fmax-5cts.vsz
    % PATH = /home/steff075/phd_ecm/IRAS13224-3809/IRAS13224-lag-results-All-fmax.vsz
    \includegraphics*[scale=0.43]{images/1H0707-lag-results-All-fmax-5cts-FP.pdf}\\[4pt]
    \includegraphics*[scale=0.43]{images/IRAS-lag-results-All-fmax-FP2.pdf}
    \caption{Combination plots for the lag-frequency groups for 1H~0707-495 \emph{(top panels)} and IRAS~13224-3809 \emph{(bottom panels)} calculated to the maximum frequency $\nu_{max}$ for each source. For clarity, these plots are presented individually in HYC22.}
    \label{fig:lo_hi_lags}
\end{figure}

\begin{figure}
    \centering
    % PATH = /home/steff075/phd_ecm/1h0707/1H0707-lag-results-lo-hi-2.vsz
    \includegraphics*[scale=0.36]{images/1H0707-lag-results-lo-med-hi-2.pdf}
    \caption{The lag-frequency groups for 1H~0707-495 showing the high-counts group (red), medium-counts (orange) and low-counts (green). The combined time lags are shown in black.}
    \label{fig:1h_lags}
\end{figure}


\begin{figure}
    \centering
    % PATH = PATH /home/steff/phd_ecm/IRAS13224-3809/lag-results-lo-hi-flux.vsz
    \includegraphics*[scale=0.45]{images/IRAS-lag-results-lo-hi-flux.pdf}
    \caption{IRAS13224-3809 lag frequency for the spectral groups outlined in the text above.}
    \label{fig:IRAS_lags}
\end{figure}


\begin{table}
\centering
\caption[ECM fits]{The extended corona results for 1H 0707-495 fitted to $90\%$ confidence.} 
\label{1H_ecm_results}
\begin{tabular}{cccccccccc}
\hline
{Obs Id} & {$\chi^2 / \text{DoF}$}  & {$log M M_\odot$} & {$h_2$} & {$\Gamma_1$}  & {$\Gamma_2$} & {$\xi$} & {$b$} & {$t_\text{max}$} & {$t_\text{shift}$}\\
\hline
Combined & 2.04 & $6.03^{+0.02}_{-0.02}$ & $3.00^{+0.03}_{-0.19}$ & $3.0^{+0.00}_{-0.00}$ & $2.9^{+0.00}_{-0.19}$ & $3.0^{+0.00}_{-0.00}$	& $2.00^{+0.00}_{-0.00}$ & $569.00^{+0.00}_{-48.52}$ & $91.00^{+10.06}_{-0.00}$ \\
Hi-flux & 3.34 & $5.94^{+0.04}_{-0.04}$ & $4.00^{+0.00}_{-0.00}$ & $1.7^{+0.00}_{-0.00}$ & $1.4^{+0.00}_{-0.00}$ & $1.0^{+0.00}_{-0.00}$	& $1.00^{+0.00}_{-0.00}$ & $490.00^{+0.00}_{-206.32}$ & $65.00^{+0.00}_{-7.97}$ \\
Hi $(>20$~cts~$s^{-1})$ & 2.43 & $5.99^{+0.03}_{-0.03}$ & $5.00^{+0.00}_{-0.00}$ & $1.9^{+0.00}_{-0.00}$ & $1.6^{+0.00}_{-0.00}$ & $0.0^{+0.00}_{-0.00}$	& $1.00^{+0.81}_{-0.00}$ & $500.00^{+0.00}_{-168.65}$ & $90.00^{+0.00}_{-72.19}$ \\
Med-flux & 0.27 & $5.93^{+0.16}_{-0.08}$ & $6.00^{+0.00}_{-2.16}$ & $2.8^{+0.00}_{-0.00}$ & $2.4^{+0.00}_{-0.00}$ & $2.0^{+0.00}_{-0.00}$	& $2.00^{+0.00}_{-0.00}$ & $100.00^{+0.46}_{-1.54}$ & $60.00^{+0.23}_{-0.77}$ \\
Lo-flux & 1.59 & $6.14^{+0.05}_{-0.04}$ & $6.00^{+0.00}_{-0.00}$ & $3.3^{+0.00}_{-0.69}$ & $2.9^{+0.00}_{-0.00}$ & $1.0^{+0.00}_{-0.00}$	& $1.00^{+0.00}_{-0.00}$ & $250.00^{+88.28}_{-121.22}$ & $10.00^{+21.79}_{-0.00}$ \\
Lo $(<20$~cts~$s^{-1})$ & 0.95 & $6.26^{+0.02}_{-0.02}$ & $5.00^{+0.00}_{-0.00}$ & $3.0^{+0.10}_{-0.00}$ & $2.6^{+0.22}_{-0.00}$ & $0.0^{+0.00}_{-0.00}$	& $2.00^{+0.00}_{-0.00}$ & $210.00^{+36.55}_{-0.00}$ & $17.00^{+3.38}_{-15.94}$ \\
0110890201 & 0.08 &	$6.03^{+0.12}_{-0.03}$ & $7.00^{+0.00}_{-1.00}$ & $3.1^{+0.00}_{-0.00}$ & $2.9^{+0.00}_{-0.02}$ & $3.00^{+0.00}_{-0.00}$	& $3.00^{+0.00}_{-0.00}$ & $560.00^{+5.14}_{-27.55}$ & $20.00^{+1.37}_{-2.21}$ \\
0148010301 & 0.96 & $6.21^{+0.06}_{-0.07}$ & $5.00^{+2.67}_{-0.00}$ & $2.4^{+0.00}_{-0.00}$ & $2.2^{+0.75}_{-0.00}$ & $2.00^{+0.00}_{-0.00}$	& $3.00^{+0.00}_{-0.00}$ & $700.00^{+25.57}_{-44.73}$ & $60.00^{+0.00}_{-4.06}$ \\
0506200201 & 1.17 &	$6.15^{+0.06}_{-0.04}$ & $5.00^{+0.00}_{-0.00}$ & $3.0^{+0.00}_{-0.00}$ & $2.9^{+0.00}_{-0.00}$ & $0.00^{+0.00}_{-0.00}$	& $1.00^{+0.00}_{-0.00}$ & $500.00^{+0.00}_{-0.00}$ & $85.00^{+0.00}_{-31.60}$ \\
0506200301 & 1.31 &	$5.99^{+0.11}_{-0.08}$ & $3.00^{+0.00}_{-0.00}$ & $2.5^{+0.00}_{-0.00}$ & $2.3^{+0.00}_{-0.00}$ & $3.00^{+0.00}_{-0.00}$	& $3.00^{+0.00}_{-0.00}$ & $250.00^{+0.00}_{-0.00}$ & $80.00^{+35.34}_{-77.88}$ \\
0506200401 & 1.11 &	$6.13^{+0.16}_{-0.19}$ & $3.00^{+0.00}_{-0.00}$ & $2.6^{+0.00}_{-0.00}$ & $2.0^{+0.84}_{-0.00}$ & $0.00^{+0.00}_{-0.00}$	& $1.00^{+0.00}_{-0.00}$ & $600.00^{+0.00}_{-0.00}$ & $110.00^{+0.00}_{-0.00}$ \\
0506200501 & 0.95 &	$6.47^{+0.06}_{-0.09}$ & $3.00^{+0.00}_{-0.00}$ & $3.0^{+0.06}_{-0.00}$ & $1.7^{+1.13}_{-0.00}$ & $3.00^{+0.00}_{-0.00}$	& $2.00^{+0.00}_{-0.00}$ & $350.00^{+0.00}_{-241.21}$ & $120.00^{+0.00}_{-0.00}$ \\
0511580101 & 0.24 & $6.24^{+0.04}_{-0.06}$ & $6.00^{+0.00}_{-0.00}$ & $2.6^{+0.00}_{-0.00}$ & $2.2^{+0.00}_{-0.00}$ & $1.00^{+0.00}_{-0.00}$	& $2.00^{+0.00}_{-0.00}$ & $250.00^{+434.73}_{-72.45}$ & $20.00^{+99.30}_{-0.00}$ \\
0511580201 & 1.25 &	$6.40^{+0.06}_{-0.10}$ & $8.00^{+0.00}_{-0.00}$ & $2.8^{+0.28}_{-0.04}$ & $2.0^{+0.00}_{-0.00}$ & $1.00^{+0.00}_{-0.00}$	& $1.00^{+0.00}_{-0.00}$ & $150.00^{+313.42}_{-0.00}$ & $30.00^{+64.62}_{-27.31}$ \\
0511580301 & 0.95 &	$6.32^{+0.03}_{-0.02}$ & $16.00^{+0.00}_{-3.88}$ & $2.8^{+0.00}_{-0.39}$ & $2.1^{+0.00}_{-0.00}$ & $3.00^{+0.00}_{-0.00}$	& $3.00^{+0.00}_{-0.63}$ & $250.00^{+6.59}_{-0.23}$ & $20.00^{+1.09}_{-7.60}$ \\
0511580401 & 0.66 &	$6.40^{+0.05}_{-0.02}$ & $3.00^{+0.00}_{-0.00}$ & $2.6^{+0.00}_{-0.00}$ & $2.4^{+0.00}_{-0.00}$ & $1.00^{+0.00}_{-0.00}$	& $3.00^{+0.00}_{-0.00}$ & $300.00^{+0.00}_{-0.00}$ & $50.00^{+0.00}_{-47.76}$ \\
0554710801 & 1.78 &	$6.19^{+0.09}_{-0.06}$ & $3.00^{+0.00}_{-0.00}$ & $3.0^{+0.02}_{-0.68}$ & $2.3^{+0.00}_{-0.00}$ & $0.00^{+0.00}_{-0.00}$	& $2.00^{+0.00}_{-0.02}$ & $100.00^{+176.69}_{-0.00}$ & $10.00^{+68.17}_{-7.93}$ \\
0653510301 & 0.65 &	$6.26^{+0.08}_{-0.07}$ & $5.00^{+0.00}_{-0.00}$ & $2.3^{+0.00}_{-0.00}$ & $2.2^{+0.35}_{-0.00}$ & $2.00^{+0.00}_{-0.00}$	& $3.00^{+0.00}_{-0.00}$ & $700.00^{+0.00}_{-0.00}$ & $80.00^{+0.00}_{-41.95}$ \\
0653510401 & 0.09 &	$6.01^{+0.06}_{-0.03}$ & $5.00^{+2.59}_{-0.00}$ & $2.2^{+0.00}_{-0.00}$ & $2.0^{+0.35}_{-0.00}$ & $2.00^{+0.00}_{-0.00}$	& $2.00^{+0.00}_{-0.02}$ & $480.00^{+48.67}_{-218.72}$ & $50.00^{+11.61}_{-26.76}$ \\
0653510501 & 1.64 &	$6.01^{+0.02}_{-0.07}$ & $19.00^{+0.00}_{-14.42}$ & $2.5^{+0.00}_{-0.00}$ & $1.8^{+0.00}_{-0.00}$ & $1.00^{+0.00}_{-0.00}$	& $3.00^{+0.00}_{-0.00}$ & $400.00^{+18.20}_{-3.44}$ & $20.00^{+14.67}_{-18.22}$ \\
0653510601 & 1.69 &	$5.91^{+0.06}_{-0.06}$ & $5.00^{+0.00}_{-0.00}$ & $3.0^{+0.00}_{-0.05}$ & $2.8^{+0.34}_{-0.00}$ & $2.00^{+0.00}_{-0.00}$	& $2.00^{+0.00}_{-0.02}$ & $520.00^{+0.00}_{-225.70}$ & $30.00^{+59.26}_{-10.17}$ \\ \hline 
\end{tabular}
\end{table}


\begin{table}
\centering
\caption[ECM fits]{The extended corona results for IRAS 13224-3809 individual observations fitted to $90\%$ confidence.} 
\label{IRAS_ecm_results}
\begin{tabular}{cccccccccc}
\hline
{Obs Id} & {$\chi^2 / \text{DoF}$}  & {$log M M_\odot$} & {$h_2$} & {$\Gamma_1$}  & {$\Gamma_2$} & {$\xi$} & {$b$} & {$t_\text{max}$} & {$t_\text{shift}$}\\
\hline
Combined & 7.85 & $6.10^{+00}_{00}$ & $5.00^{+6.19}_{-0.00}$ & $2.4^{+0.00}_{-0.00}$ & $2.3^{+0.32}_{-0.00}$ & $3.0^{+0.00}_{-0.00}$	& $1.00^{+0.00}_{-0.00}$ & $1000.00^{+0.00}_{-319.21}$ & $110.00^{+0.00}_{-64.57}$ \\
Hi-flux & 3.16 & $6.09^{+00}_{00}$ & $6.00^{+0.00}_{-0.00}$ & $2.0^{+0.00}_{-0.00}$ & $1.8^{+0.00}_{-0.19}$ & $3.0^{+0.00}_{-0.00}$	& $1.00^{+0.00}_{-0.00}$ & $1100.00^{+0.00}_{-405.29}$ & $120.00^{+0.00}_{-0.00}$ \\
Hi $(>20$~cts~$s^{-1})$ & 2.61 & $6.11^{+00}_{00}$ & $5.00^{+0.00}_{-0.00}$ & $2.3^{+0.00}_{-0.12}$ & $2.1^{+0.00}_{-0.19}$ & $0.0^{+0.00}_{-0.00}$	& $1.00^{+0.06}_{-0.00}$ & $1000.00^{+0.00}_{-317.73}$ & $110.00^{+0.00}_{-24.9}$ \\
Med-flux & 2.61 & $6.09^{+00}_{00}$ & $5.00^{+0.00}_{-0.00}$ & $2.4^{+0.00}_{-0.00}$ & $2.3^{+0.00}_{-0.69}$ & $3.0^{+0.00}_{-0.00}$	& $1.00^{+0.00}_{-0.00}$ & $1000.00^{+0.00}_{-303.86}$ & $60.00^{+29.57}_{-53.03}$ \\
Lo-flux & 6.45 & $5.83^{+00}_{00}$ & $6.00^{+0.59}_{-1.02}$ & $2.4^{+0.19}_{-0.11}$ & $2.3^{+0.04}_{-0.11}$ & $1.0^{+0.00}_{-0.00}$	& $3.00^{+0.00}_{-0.00}$ & $1000.00^{+39.87}_{-44.43}$ & $40.00^{+3.98}_{-10.57}$ \\
Lo $(<20$~cts~$s^{-1})$ & 4.24 & $6.07^{+00}_{00}$ & $8.00^{+0.00}_{-0.00}$ & $2.7^{+0.00}_{-0.12}$ & $2.6^{+0.00}_{-0.00}$ & $3.0^{+0.00}_{-0.00}$	& $1.00^{+0.00}_{-0.00}$ & $1200.00^{+0.00}_{-406.42}$ & $70.00^{+0.14}_{-51.99}$ \\
0110890101 & 1.04 &	$6.28^{+0.02}_{-0.02}$ & $18.00^{+0.00}_{-14.26}$ & $2.3^{+0.00}_{-0.00}$ & $1.8^{+0.00}_{-0.02}$ & $3.00^{+0.00}_{-0.00}$	& $3.00^{+0.00}_{-0.00}$ & $700.00^{+0.00}_{-228.16}$ & $40.00^{+25.45}_{-39.46}$ \\
0673580101 & 0.22 & $6.84^{+0.03}_{-0.03}$ & $3.00^{+0.00}_{-0.00}$ & $2.6^{+0.00}_{-0.00}$ & $1.8^{+0.00}_{-0.00}$ & $1.00^{+0.00}_{-0.00}$	& $3.00^{+0.00}_{-0.00}$ & $500.00^{+0.00}_{-0.00}$ & $10.00^{+0.00}_{-0.00}$ \\
0673580201 & 0.14 &	$6.28^{+0.08}_{-0.10}$ & $4.00^{+0.00}_{-0.00}$ & $2.6.0^{+0.00}_{-0.00}$ & $2.4^{+0.00}_{-0.00}$ & $3.00^{+0.00}_{-0.00}$	& $2.00^{+0.00}_{-0.00}$ & $400.00^{+0.00}_{-296.52}$ & $30.00^{+0.00}_{-0.00}$ \\
0673580301 & 0.16 &	$6.51^{+0.06}_{-0.06}$ & $3.00^{+0.00}_{-0.00}$ & $2.7^{+0.00}_{-0.00}$ & $2.4^{+0.00}_{-0.00}$ & $3.00^{+0.00}_{-0.00}$	& $1.00^{+0.00}_{-0.00}$ & $200.00^{+0.00}_{-0.00}$ & $30.00^{+0.00}_{-13.64}$ \\
0673580401 & 2.52 &	$6.41^{+0.04}_{-0.06}$ & $13.00^{+0.00}_{-2.22}$ & $2.3^{+0.00}_{-0.00}$ & $1.8^{+0.00}_{-0.00}$ & $2.00^{+0.00}_{-0.00}$	& $3.00^{+0.00}_{-0.00}$ & $500.00^{+292.25}_{-117.44}$ & $20.00^{+20.82}_{-0.04}$ \\
0780560101 & 0.49 &	$6.45^{+0.10}_{-0.10}$ & $20.00^{+0.00}_{-0.00}$ & $2.4^{+0.00}_{-0.00}$ & $1.9^{+0.00}_{-0.00}$ & $3.00^{+0.00}_{-0.00}$	& $3.00^{+0.00}_{-0.00}$ & $600.00^{+0.00}_{-478.29}$ & $40.00^{+0.00}_{-0.00}$ \\
0780561301 & 0.55 & $6.35^{+0.04}_{-0.05}$ & $3.00^{+0.00}_{-0.00}$ & $2.7^{+0.00}_{-0.00}$ & $2.5^{+0.00}_{-0.00}$ & $3.00^{+0.00}_{-0.00}$	& $3.00^{+0.00}_{-1.56}$ & $700.00^{+0.00}_{-213.69}$ & $30.00^{+25.91}_{-17.59}$ \\
0780561401 & 2.01 &	$6.73^{+0.04}_{-0.04}$ & $16.00^{+0.00}_{-0.00}$ & $2.4^{+0.00}_{-0.00}$ & $1.8^{+0.00}_{-0.00}$ & $2.00^{+0.00}_{-0.00}$	& $3.00^{+0.00}_{-0.00}$ & $300.00^{+0.00}_{-23.42}$ & $20.00^{+17.77}_{-0.00}$ \\
0780561501 & 4.09 &	$5.48^{+0.00}_{-0.00}$ & $16.00^{+0.00}_{-0.00}$ & $2.6^{+0.00}_{-0.00}$ & $2.5^{+0.00}_{-0.00}$ & $1.00^{+0.00}_{-0.00}$	& $1.00^{+0.00}_{-0.00}$ & $1200.00^{+0.00}_{-0.00}$ & $100.00^{+0.00}_{-0.00}$ \\
0780561601 & 3.82 &	$6.14^{+0.00}_{-0.00}$ & $5.00^{+2.41}_{-0.00}$ & $2.4^{+0.00}_{-0.00}$ & $2.3^{+0.00}_{-0.00}$ & $1.00^{+0.00}_{-0.00}$	& $3.00^{+0.00}_{-0.00}$ & $1000.00^{+0.00}_{-211.35}$ & $20.00^{+17.65}_{-2.68}$ \\
0780561701 & 0.26 &	$6.28^{+0.13}_{-0.04}$ & $6.00^{+0.00}_{-0.00}$ & $2.2^{+0.00}_{-0.00}$ & $1.9^{+0.00}_{-0.00}$ & $3.00^{+0.00}_{-0.00}$	& $1.00^{+0.00}_{-0.00}$ & $1200.00^{+0.00}_{-0.00}$ & $100.00^{+0.00}_{-0.00}$ \\
0792180101 & 0.54 &	$6.38^{+0.07}_{-0.07}$ & $17.00^{+0.00}_{-0.00}$ & $2.4^{+0.00}_{-0.00}$ & $1.7^{+0.00}_{-0.00}$ & $3.00^{+0.00}_{-0.00}$	& $3.00^{+0.00}_{-0.00}$ & $500.00^{+0.00}_{-212.52}$ & $20.00^{+0.00}_{-0.00}$ \\
0792180201 & 0.52 &	$6.22^{+0.05}_{-0.05}$ & $20.00^{+0.00}_{-0.00}$ & $2.4^{+0.00}_{-0.00}$ & $1.9^{+0.00}_{-0.00}$ & $2.00^{+0.00}_{-0.00}$	& $2.00^{+0.00}_{-0.00}$ & $400.00^{+0.00}_{-200.21}$ & $30.00^{+0.00}_{-0.00}$ \\
0792180301 & 0.33 &	$6.50^{+0.03}_{-0.02}$ & $16.00^{+0.00}_{-6.61}$ & $2.7^{+0.00}_{-0.59}$ & $2.1^{+0.00}_{-0.00}$ & $1.00^{+0.00}_{-0.00}$	& $3.00^{+0.00}_{-1.17}$ & $300.00^{+310.62}_{-26.44}$ & $20.00^{+4.50}_{-5.01}$ \\
0792180401 & 1.26 &	$6.36^{+0.04}_{-0.05}$ & $20.00^{+0.00}_{-8.38}$ & $2.9^{+0.00}_{-0.00}$ & $2.4^{+0.00}_{-0.00}$ & $3.00^{+0.00}_{-0.00}$	& $3.00^{+0.00}_{-0.00}$ & $1000.00^{+0.00}_{-767.15}$ & $20.00^{+9.84}_{-5.43}$ \\ 
0792180501 & 0.75 &	$6.33^{+0.07}_{-0.07}$ & $16.00^{+0.00}_{-0.00}$ & $2.8^{+0.00}_{-0.00}$ & $2.3^{+0.00}_{-0.00}$ & $1.00^{+0.00}_{-0.00}$	& $3.00^{+0.00}_{-0.00}$ & $500.00^{+0.00}_{-0.00}$ & $20.00^{+16.25}_{-0.00}$ \\ 
0792180601 & 0.62 &	$6.27^{+0.06}_{-0.12}$ & $3.00^{+0.00}_{-0.00}$ & $2.2^{+0.00}_{-0.00}$ & $1.9^{+0.00}_{-0.00}$ & $2.00^{+0.00}_{-0.00}$	& $1.00^{+0.00}_{-0.00}$ & $600.00^{+0.00}_{-339.56}$ & $90.00^{+0.00}_{-0.00}$ \\ 
\hline 
\end{tabular}
\end{table}



\begin{comment}
\onecolumn
\begin{figure}
\centering
% PATH = PATH /home/steff/phd_ecm/1h0707/lightcurves/1H0707_multi_lc_plots3.vsz
    \includegraphics*[scale=0.55]{images/1H0707_multi_lc_plots_ALL.pdf}
    \caption{1H~0707-495 light curves in the 0.3 -- 10 keV energy range for each of the individual observations with the ID numbers above each data set, the x-axis is not to scale and some labels have been removed for clarity.}
    \label{fig:1h_lightcuvres2}
\end{figure}

\begin{table}
\centering
\caption[Relxill spectral fits]{Results for 1H 0707-495 groupings detailing the model flux, soft (reverberation) lag and frequency where the largest soft lags were found. The best \texttt{RELXILL} model spectral fits are also included to $90\%$ confidence.} 
\label{1H_spec_results}
\begin{tabular}{cccccccccc}
\hline
{Group} & Flux (0.3 - 10~keV) & Soft Lag & Frequency & {$\Gamma_\texttt{Relxill}$}  & {$\log \xi$} & {$AF_e$} & {RF} & {\textit{i}} & {$\chi^2$ / DoF}\\ 
& (erg cm$^{-2}$ s $^{-1}$) & (s) & (Hz) &  &  &  &  & & \\ \hline 
Comb & 2.91 $\times~10^{-12}$ & $26.6 \pm~2.9$ & 1.61 $\times~10^{-3}$ & $3.38^{+0.02}_{-0.01}$ & $2.37^{+0.05}_{-0.05}$ & $0.50^{+0.05}_{-0.00}$ & $10.00^{+0.00}_{-0.10}$ & $74.90^{+0.99}_{-1.52}$ & 1533/683 \\ [3pt]
Hi & 3.40 $\times~10^{-12}$ & $26.6 \pm~3.0$ & 1.61 $\times~10^{-3}$  & $3.40^{+0.00}_{-0.02}$  &  $2.43^{+0.06}_{-0.05}$ & $0.50^{+0.04}_{-0.00}$ & $10.00^{+0.00}_{-0.08}$ & $76.68^{+0.69}_{-1.04}$ & 1382/646\\ [3pt]
Hi > 20 cts~s$^{-1}$ & 2.80 $\times~10^{-12}$ & $32.5 \pm~3.9$ & 1.61 $\times~10^{-3}$  & $3.40^{+0.00}_{-0.02}$  &  $2.43^{+0.06}_{-0.05}$ & $0.50^{+0.01}_{-0.00}$ & $10.00^{+0.00}_{-0.08}$ & $76.93^{+0.83}_{-1.45}$ & 995/690\\ [3pt]
Med & 3.28 $\times~10^{-14}$ & $35.7 \pm~9.6$ & 1.61 $\times~10^{-3}$  & $2.80^{+0.14}_{-0.34}$ &  $3.58^{+0.16}_{-0.32}$ & $10.00^{+0.00}_{-1.64}$ & $10.00^{+0.00}_{-4.90}$ & $76.10^{+1.09}_{-0.75}$ & 446/411 \\ [3pt]
Lo & 4.07 $\times~10^{-14}$ & $28.7 \pm~10.5$ & 1.61 $\times~10^{-3}$  & $2.73^{+0.12}_{-0.16}$ &  $2.85^{+0.18}_{-0.15}$ & $9.59^{+0.41}_{-0.49}$ & $10.00^{+0.00}_{-1.17}$ & $80.00^{+0.00}_{-2.99}$ & 539/437  \\ [3pt]
Lo < 20 cts~s$^{-1}$ & 9.15 $\times~12^{-13}$ & $23.5 \pm~11.7$ & 5.86 $\times~10^{-4}$  & $3.38^{+0.01}_{-0.04}$ &  $2.43^{+0.07}_{-0.07}$ & $0.50^{+0.06}_{-0.00}$ & $10.00^{+0.00}_{-0.13}$ & $80.00^{+0.00}_{-2.99}$ & 1251/680\\ \hline 
\end{tabular}
\end{table}
\end{comment}


\twocolumn


\begin{comment}
\begin{table}
\caption{Results of the extended corona model fitted to four combined spectral states of the lag-frequency of 1H~0707-495.}
    \label{1h_fitsN}
    \begin{tabular}{lrrrr}
        \hline
        {Parameter} & {Comb} &  {Low} &  {Medium} &  {High}\\  
        \\ \hline \\ 
        $h_2$ & $3.00^{+0.03}_{-0.19}$ & $6.00^{+0.00}_{-0.00}$ & $6.00^{+0.00}_{-2.16}$ & $4.00^{+0.00}_{-0.00}$\\ [1ex]  
        $\Gamma_1$ & $3.00^{+0.00}_{-0.00}$ &  $3.30^{+0.00}_{-0.69}$ & $2.80^{+0.00}_{-0.00}$ & $1.70^{+0.00}_{-0.00}$\\ [1ex] 
        $\Gamma_2$ & $2.90^{+0.00}_{-0.19}$ &  $2.90^{+0.00}_{-0.00}$  & $2.40^{+0.00}_{-0.00}$ & $1.47^{+0.00}_{-0.00}$\\ [1ex]  
        $\xi$ &  $3.00^{+0.20}_{-0.07}$ &  $1.00^{+0.00}_{-0.00}$  & $2.00^{+0.00}_{-0.00}$ & $1.00^{+0.00}_{-0.00}$\\ [1ex]  
        $b$ & $2.00^{+0.00}_{-0.00}$ & $1.00^{+0.00}_{-0.00}$ & $2.00^{+0.00}_{-0.00}$ & $1.00^{+1.72}_{-0.00}$\\ [1ex]  
        $t_\text{max}$  &  $569^{+0.00}_{-48.52}$ &  $250^{+88.28}_{-121.22}$ & $100.00^{+0.46}_{-1.54}$ & $490.00^{+0.00}_{-206.32}$\\ [1ex]  
        $t_\text{shift}$ & $91^{+10.06}_{-~0.00}$ & $10.00^{+21.79}_{-0.00}$  & $60.00^{+0.23}_{-0.77}$ & $65.00^{+0.00}_{-9.97}$\\ [1ex]
        log $M$ & $6.03^{+0.02}_{-0.02}$ & $6.14^{+0.05}_{-0.04}$ & $5.93^{+0.16}_{-0.08}$ & $5.94^{+0.04}_{-0.04}$\\ [1ex]
        \hline  
        {$\chi^2 / \text{d.o.f}$} & {2.04} &  {1.59} & {0.27} & {3.34}\\  \hline 
    \end{tabular}
\end{table}
\end{comment}


%\onecolumn
%\begin{figure}
%    \centering
    % PATH = PATH /home/steff/phd_ecm/IRAS13224-3809/lightcurves/IRAS13224_multi_lc_plots3.vsz
%    \includegraphics*[scale=0.55]{images/IRAS_multi_lc_plots_ALL.pdf}
%    \caption{IRAS13224-3809 light curves in the 0.3 -- 10 keV energy range for each of the individual observations with the ID numbers centred above each data set, the x-axis is not to scale and some labels have been removed for clarity.}
%    \label{fig:IRAS_lightcuvres}
%\end{figure}


\begin{comment}
\begin{table}
\centering
\caption[Relxill spectral fits]{Results for IRAS 13224-3809 groupings detailing the model flux, soft (reverberation) lag and frequency where the largest soft lags were found. The best \texttt{RELXILL} model spectral fits are also included as computed to $90\%$ confidence.} 
\label{IRAS_spec_results}
\begin{tabular}{cccccccccc}
\hline
{Group} & Flux (0.3 - 10~keV)  & Soft Lag & Frequency & {$\Gamma_\texttt{Relxill}$}  & {$\log \xi$} & {$AF_e$} & {RF} & {\textit{i}} & {$\chi^2$ / DoF}\\ 
& (erg cm$^{-2}$ s $^{-1}$) & (s) & (Hz) &  &  &  &  & & \\ \hline 
Comb & $1.81 \times10^{-12}$ & $ 49.7 \pm 10.5$  & $ 4.36 \times 10^{-4}$ & $3.25^{+0.04}_{-0.02}$ & $2.13^{+0.06}_{-0.06}$ & $0.50^{+0.11}_{-0.00}$ & $10.00^{+0.00}_{-1.80}$ & $77.51^{+1.39}_{-1.18}$ & 2199/1281 \\ [3pt]
Hi & $ 3.46 \times 10^{-12}$ & $67.3 \pm 26.0$ & $ 4.36 \times 10^{-4}$ & $3.17^{+0.09}_{-0.08}$ & $1.41^{+0.40}_{-0.10}$ & $2.79^{+1.40}_{-2.02}$ & $9.08^{+0.91}_{-0.92}$ & $77.82^{+2.18}_{-2.19}$ & 1237/1000\\[3pt]
Hi $>20$~cts~s$^{-1}$ & $ 1.81 \times 10^{-12}$ & $50.8 \pm 15.9$ & $ 4.36 \times 10^{-4}$ & $3.06^{+0.06}_{-0.04}$ & $1.46^{+0.17}_{-0.08}$ & $0.50^{+0.41}_{-0.00}$ & $10.00^{+0.00}_{-0.61}$ & $79.91^{+0.09}_{-2.82}$ & 1558/1353\\[3pt]
Med & $ 1.41 \times 10^{-12}$ & $35.2 \pm 12.2$ & $ 4.36 \times 10^{-4}$ & $3.27^{+0.00}_{-0.00}$ & $2.12^{+0.01}_{-0.00}$ & $0.86^{+0.02}_{-0.00}$ & $10.00^{+0.00}_{-0.03}$ & $72.30^{+0.34}_{-0.40}$ & 1699/1455\\[3pt]
Lo & $5.18 \times 10^{-13}$ & $76.4 \pm~34.2$ & $4.36 \times 10^{-4}$ & $3.14^{+0.06}_{-0.21}$ & $1.88^{+0.17}_{-0.13}$ & $0.50^{+0.71}_{-0.00}$ & $10.00^{+0.00}_{-0.75}$ & $65.46^{+3.35}_{-2.32}$ & 834/799 \\ [3pt]
Lo $>20$~cts~s$^{-1}$ & $1.45 \times 10^{-12}$ & $41.7 \pm~14.4$ & $4.36 \times 10^{-4}$ & $3.16^{+0.03}_{-0.04}$ & $1.83^{+0.06}_{-0.08}$ & $0.50^{+0.10}_{-0.00}$ & $10.00^{+0.00}_{-0.02}$ & $74.69^{+1.09}_{-1.41}$ & 1579/1275 \\ \hline \end{tabular}
\end{table}
\end{comment}

\begin{table*}
\centering
\caption[ECM fits]{The initial variable-mass extended corona results for 1H 0707-495 fitted to $90\%$ confidence (from the \texttt{BlueCrystal} phase).} 
\label{1H_ecm_results}
\begin{tabular}{cccccccccc}
\hline
{Obs Id} & {$\chi^2 / \text{DoF}$}  & {$log M M_\odot$} & {$h_2$} & {$\Gamma_1$}  & {$\Gamma_2$} & {$\xi$} & {$b$} & {$t_\text{max}$} & {$t_\text{shift}$}\\
\hline
Combined & 2.32 & $6.22^{+0.01}_{-0.01}$ & $20.00^{+0.00}_{-0.11}$ & $2.6^{+0.00}_{-0.07}$ & $2.1^{+0.72}_{-0.00}$ & $3.0^{+0.00}_{-0.00}$	& $2.00^{+0.00}_{-0.00}$ & $250.00^{+67.82}_{-0.00}$ & $20.00^{+11.05}_{-11.92}$   \\[3pt] 
Hi-flux  & 2.35 & $6.26^{+0.01}_{-0.01}$ & $11.00^{+1.83}_{-3.79}$ & $2.5^{+0.00}_{-0.26}$ & $1.7^{+0.83}_{-0.00}$ & $3.0^{+0.00}_{-0.00}$	& $1.00^{+0.00}_{-0.00}$ & $200.00^{+125.32}_{-90.09}$ & $20.00^{+11.75}_{-14.48}$ \\[3pt]
Hi $>20$~cts~s$^{-1}$ & 1.01 & $6.33^{+0.02}_{-0.01}$ & $20.00^{+0.00}_{-1.48}$ & $3.0^{+0.00}_{-0.67}$ & $2.4^{+0.04}_{-0.68}$ & $3.0^{+0.00}_{-0.00}$	& $3.00^{+0.00}_{-0.55}$ & $250.00^{+3.61}_{-12.31}$ & $20.00^{+5.38}_{-6.36}$ \\ [3pt]
Med-flux & 1.19 & $5.84^{+0.06}_{-0.07}$ & $3.00^{+0.00}_{-0.00}$ & $2.2^{+0.00}_{-0.00}$ & $2.0^{+0.00}_{-0.00}$ & $1.0^{+0.00}_{-0.00}$	& $1.00^{+0.00}_{-0.00}$ & $200.00^{+0.00}_{-109.26}$ & $100.00^{+0.00}_{-36.88}$ \\[3pt]
Lo-flux & 0.74 & $6.25^{+0.05}_{-0.10}$ & $8.00^{+0.00}_{-0.00}$ & $2.8^{+0.00}_{-0.00}$ & $2.3^{+0.00}_{-0.00}$ & $1.0^{+0.00}_{-0.00}$	& $1.00^{+0.00}_{-0.00}$ & $220.00^{+0.00}_{-0.00}$ & $50.00^{+0.00}_{-0.00}$ \\[3pt]
Lo $<20$~cts~s$^{-1}$ & 0.21 & $6.15^{+0.02}_{-0.02}$ & $16.00^{+0.00}_{-0.00}$ & $2.6^{+0.00}_{-0.00}$ & $1.7^{+0.00}_{-0.00}$ & $3.0^{+0.00}_{-0.00}$	& $1.00^{+0.00}_{-0.00}$ & $250.00^{+0.00}_{-0.00}$ & $20.00^{+0.53}_{-0.00}$ \\[3pt]
0110890201 & 2.24 &	$5.90^{+0.14}_{-0.06}$ & $4.00^{+0.00}_{-0.00}$ & $2.6^{+0.00}_{-0.00}$ & $2.5^{+0.00}_{-0.00}$ & $0.00^{+0.00}_{-0.00}$	& $2.00^{+0.00}_{-0.00}$ & $600.00^{+0.00}_{-0.00}$ & $50.00^{+0.00}_{-0.00}$ \\[3pt]
0148010301 & 1.52 & $6.32^{+0.03}_{-0.03}$ & $12.00^{+0.00}_{-0.00}$ & $2.8^{+0.00}_{-0.00}$ & $2.3^{+0.00}_{-0.00}$ & $1.00^{+0.00}_{-0.00}$	& $2.00^{+0.00}_{-0.00}$ & $700.00^{+8.46}_{-0.00}$ & $30.00^{+0.00}_{-0.00}$ \\[3pt]
0506200201 & 0.19 &	$6.45^{+0.05}_{-0.03}$ & $5.00^{+0.00}_{-0.00}$ & $2.7^{+0.00}_{-0.00}$ & $2.5^{+0.00}_{-0.00}$ & $1.00^{+0.00}_{-0.00}$	& $3.00^{+0.00}_{-0.00}$ & $400.00^{+0.00}_{-0.00}$ & $60.00^{+12.28}_{-22.54}$ \\[3pt]
0506200301 & 0.47 &	$6.17^{+0.05}_{-0.10}$ & $3.00^{+0.00}_{-0.00}$ & $2.2^{+0.00}_{-0.00}$ & $2.0^{+0.00}_{-0.00}$ & $0.00^{+0.00}_{-0.00}$	& $3.00^{+0.00}_{-0.00}$ & $500.00^{+0.00}_{-163.08}$ & $60.00^{+15.87}_{-55.83}$ \\[3pt]
0506200401 & 3.07 &	$6.54^{+0.01}_{-0.01}$ & $15.00^{+16.53}_{-5.3}$ & $2.8^{+0.00}_{-0.03}$ & $1.8^{+0.84}_{-0.00}$ & $1.00^{+0.00}_{-0.00}$	& $3.00^{+0.00}_{-0.00}$ & $400.00^{+23.81}_{-33.84}$ & $20.00^{+9.77}_{-18.96}$ \\[3pt]
0506200501 & 0.13 &	$6.85^{+0.05}_{-0.05}$ & $18.00^{+0.00}_{-0.00}$ & $3.1^{+0.00}_{-0.00}$ & $1.8^{+0.00}_{-0.00}$ & $0.00^{+0.00}_{-0.00}$	& $3.00^{+0.00}_{-0.00}$ & $450.00^{+0.00}_{-293.29}$ & $20.00^{+10.11}_{-0.00}$ \\[3pt]
0511580101 & 1.01 & $6.21^{+0.01}_{-0.02}$ & $19.00^{+0.00}_{-0.00}$ & $2.5^{+0.00}_{-0.00}$ & $2.0^{+0.00}_{-0.00}$ & $3.00^{+0.00}_{-0.00}$	& $2.00^{+0.00}_{-0.00}$ & $400.00^{+0.00}_{-221.33}$ & $30.00^{+84.41}_{-0.00}$ \\[3pt]
0511580201 & 0.48 &	$6.20^{+0.02}_{-0.04}$ & $20.00^{+0.00}_{-0.00}$ & $2.9^{+0.00}_{-0.00}$ & $1.9^{+0.00}_{-0.00}$ & $2.00^{+0.00}_{-0.00}$	& $2.00^{+0.00}_{-0.00}$ & $200.00^{+0.00}_{-0.00}$ & $10.00^{+110.50}_{-0.00}$ \\[3pt]
0511580301 & 0.63 &	$6.22^{+0.01}_{-0.01}$ & $19.00^{+0.00}_{-6.46}$ & $2.4^{+0.09}_{-0.28}$ & $1.7^{+1.01}_{-0.00}$ & $2.00^{+0.00}_{-0.00}$	& $2.00^{+0.00}_{-0.63}$ & $350.00^{+9.39}_{-6.10}$ & $30.00^{+1.58}_{-3.60}$ \\[3pt]
0511580401 & 1.22 &	$6.19^{+0.01}_{-0.01}$ & $12.00^{+0.00}_{-0.00}$ & $2.6^{+0.00}_{-0.00}$ & $2.4^{+0.00}_{-0.00}$ & $1.00^{+0.00}_{-0.00}$	& $3.00^{+0.00}_{-0.00}$ & $400.00^{+0.00}_{-162.51}$ & $120.00^{+0.00}_{-62.93}$ \\[3pt]
0554710801 & 3.84 &	$6.23^{+0.02}_{-0.02}$ & $15.00^{+0.00}_{-0.00}$ & $3.3^{+0.00}_{-0.68}$ & $2.8^{+0.00}_{-0.00}$ & $1.00^{+0.00}_{-0.00}$	& $3.00^{+0.00}_{-0.02}$ & $250.00^{+0.00}_{-213.38}$ & $40.00^{+82.16}_{-0.00}$ \\[3pt]
0653510301 & 0.01 &	$6.27^{+0.06}_{-0.18}$ & $13.00^{+0.00}_{-0.00}$ & $2.2^{+0.00}_{-0.00}$ & $1.9^{+0.00}_{-0.00}$ & $1.00^{+0.00}_{-0.00}$	& $1.00^{+0.00}_{-0.00}$ & $350.00^{+0.00}_{-0.00}$ & $110.00^{+13.15}_{-0.00}$ \\[3pt]
0653510401 & 2.31 &	$6.24^{+0.01}_{-0.01}$ & $16.00^{+0.00}_{-2.42}$ & $2.3^{+0.00}_{-0.29}$ & $1.7^{+0.94}_{-0.00}$ & $2.00^{+0.00}_{-0.00}$	& $2.00^{+0.00}_{-0.02}$ & $350.00^{+78.49}_{-7.59}$ & $30.00^{+13.88}_{-6.06}$ \\[3pt]
0653510501 & 1.32 &	$6.16^{+0.01}_{-0.02}$ & $20.00^{+0.00}_{-9.09}$ & $2.2^{+0.00}_{-0.34}$ & $1.9^{+0.00}_{-0.00}$ & $3.00^{+0.00}_{-0.00}$	& $3.00^{+0.00}_{-0.00}$ & $350.00^{+13.82}_{-15.38}$ & $30.00^{+21.31}_{-16.68}$ \\[3pt]
0653510601 & 1.19 &	$6.27^{+0.06}_{-0.05}$ & $15.00^{+0.00}_{-0.00}$ & $3.3^{+0.00}_{-1.25}$ & $1.8^{+1.31}_{-0.00}$ & $1.00^{+0.00}_{-0.00}$	& $1.00^{+0.00}_{-0.00}$ & $250.00^{+0.00}_{-0.00}$ & $40.00^{+0.00}_{-21.38}$ \\ \hline 
\end{tabular}
\end{table*}

\begin{table}
\centering
\caption[ECM fits]{The variable-mass extended corona results for IRAS 13224-3809 individual observations fitted to $90\%$ confidence.} 
\label{IRAS_ecm_results}
\begin{tabular}{cccccccccc}
\hline
{Obs Id} & {$\chi^2 / \text{DoF}$}  & {$log M M_\odot$} & {$h_2$} & {$\Gamma_1$}  & {$\Gamma_2$} & {$\xi$} & {$b$} & {$t_\text{max}$} & {$t_\text{shift}$}\\
\hline
Combined & 7.85 & $6.10^{+0.01}_{-0.01}$ & $5.00^{+6.19}_{-0.00}$ & $2.4^{+0.00}_{-0.00}$ & $2.3^{+0.32}_{-0.00}$ & $3.0^{+0.00}_{-0.00}$	& $1.00^{+0.00}_{-0.00}$ & $1000.00^{+0.00}_{-319.21}$ & $110.00^{+0.00}_{-64.57}$ \\[3pt]
Hi-flux & 3.16 & $6.09^{+0.02}_{-0.01}$ & $6.00^{+0.00}_{-0.00}$ & $2.0^{+0.00}_{-0.00}$ & $1.8^{+0.00}_{-0.19}$ & $3.0^{+0.00}_{-0.00}$	& $1.00^{+0.00}_{-0.00}$ & $1100.00^{+0.00}_{-405.29}$ & $120.00^{+0.00}_{-0.00}$ \\[3pt]
Hi $>20$~cts~s$^{-1}$ & 2.61 & $6.11^{+0.01}_{-0.02}$ & $5.00^{+0.00}_{-0.00}$ & $2.3^{+0.00}_{-0.12}$ & $2.1^{+0.00}_{-0.19}$ & $0.0^{+0.00}_{-0.00}$	& $1.00^{+0.06}_{-0.00}$ & $1000.00^{+0.00}_{-317.73}$ & $110.00^{+0.00}_{-24.9}$ \\[3pt]
Med-flux & 2.61 & $6.09^{+0.01}_{-0.01}$ & $5.00^{+0.00}_{-0.00}$ & $2.4^{+0.00}_{-0.00}$ & $2.3^{+0.00}_{-0.69}$ & $3.0^{+0.00}_{-0.00}$	& $1.00^{+0.00}_{-0.00}$ & $1000.00^{+0.00}_{-303.86}$ & $60.00^{+29.57}_{-53.03}$ \\[3pt]
Lo-flux & 6.45 & $5.83^{+0.04}_{-0.03}$ & $6.00^{+0.59}_{-1.02}$ & $2.4^{+0.19}_{-0.11}$ & $2.3^{+0.04}_{-0.11}$ & $1.0^{+0.00}_{-0.00}$	& $3.00^{+0.00}_{-0.00}$ & $1000.00^{+39.87}_{-44.43}$ & $40.00^{+3.98}_{-10.57}$ \\[3pt]
Lo $<20$~cts~s$^{-1}$ & 4.24 & $6.07^{+0.01}_{-0.02}$ & $8.00^{+0.00}_{-0.00}$ & $2.7^{+0.00}_{-0.12}$ & $2.6^{+0.00}_{-0.00}$ & $3.0^{+0.00}_{-0.00}$	& $1.00^{+0.00}_{-0.00}$ & $1200.00^{+0.00}_{-406.42}$ & $70.00^{+0.14}_{-51.99}$ \\[3pt]
0110890101 & 1.04 &	$6.28^{+0.02}_{-0.02}$ & $18.00^{+0.00}_{-14.26}$ & $2.3^{+0.00}_{-0.00}$ & $1.8^{+0.00}_{-0.02}$ & $3.00^{+0.00}_{-0.00}$	& $3.00^{+0.00}_{-0.00}$ & $700.00^{+0.00}_{-228.16}$ & $40.00^{+25.45}_{-39.46}$ \\[3pt]
0673580101 & 0.22 & $6.84^{+0.03}_{-0.03}$ & $3.00^{+0.00}_{-0.00}$ & $2.6^{+0.00}_{-0.00}$ & $1.8^{+0.00}_{-0.00}$ & $1.00^{+0.00}_{-0.00}$	& $3.00^{+0.00}_{-0.00}$ & $500.00^{+0.00}_{-0.00}$ & $10.00^{+0.00}_{-0.00}$ \\[3pt]
0673580201 & 0.14 &	$6.28^{+0.08}_{-0.10}$ & $4.00^{+0.00}_{-0.00}$ & $2.6^{+0.00}_{-0.00}$ & $2.4^{+0.00}_{-0.00}$ & $3.00^{+0.00}_{-0.00}$	& $2.00^{+0.00}_{-0.00}$ & $400.00^{+0.00}_{-296.52}$ & $30.00^{+0.00}_{-0.00}$ \\[3pt]
0673580301 & 0.16 &	$6.51^{+0.06}_{-0.06}$ & $3.00^{+0.00}_{-0.00}$ & $2.7^{+0.00}_{-0.00}$ & $2.4^{+0.00}_{-0.00}$ & $3.00^{+0.00}_{-0.00}$	& $1.00^{+0.00}_{-0.00}$ & $200.00^{+0.00}_{-0.00}$ & $30.00^{+0.00}_{-13.64}$ \\[3pt]
0673580401 & 2.52 &	$6.41^{+0.04}_{-0.06}$ & $13.00^{+0.00}_{-2.22}$ & $2.3^{+0.00}_{-0.00}$ & $1.8^{+0.00}_{-0.00}$ & $2.00^{+0.00}_{-0.00}$	& $3.00^{+0.00}_{-0.00}$ & $500.00^{+292.25}_{-117.44}$ & $20.00^{+20.82}_{-0.04}$ \\[3pt]
0780560101 & 0.49 &	$6.45^{+0.10}_{-0.10}$ & $20.00^{+0.00}_{-0.00}$ & $2.4^{+0.00}_{-0.00}$ & $1.9^{+0.00}_{-0.00}$ & $3.00^{+0.00}_{-0.00}$	& $3.00^{+0.00}_{-0.00}$ & $600.00^{+0.00}_{-478.29}$ & $40.00^{+0.00}_{-0.00}$ \\[3pt]
0780561301 & 0.55 & $6.35^{+0.04}_{-0.05}$ & $3.00^{+0.00}_{-0.00}$ & $2.7^{+0.00}_{-0.00}$ & $2.5^{+0.00}_{-0.00}$ & $3.00^{+0.00}_{-0.00}$	& $3.00^{+0.00}_{-1.56}$ & $700.00^{+0.00}_{-213.69}$ & $30.00^{+25.91}_{-17.59}$ \\[3pt]
0780561401 & 2.01 &	$6.73^{+0.04}_{-0.04}$ & $16.00^{+0.00}_{-0.00}$ & $2.4^{+0.00}_{-0.00}$ & $1.8^{+0.00}_{-0.00}$ & $2.00^{+0.00}_{-0.00}$	& $3.00^{+0.00}_{-0.00}$ & $300.00^{+0.00}_{-23.42}$ & $20.00^{+17.77}_{-0.00}$ \\[3pt]
0780561501 & 4.09 &	$5.48^{+0.00}_{-0.00}$ & $16.00^{+0.00}_{-0.00}$ & $2.6^{+0.00}_{-0.00}$ & $2.5^{+0.00}_{-0.00}$ & $1.00^{+0.00}_{-0.00}$	& $1.00^{+0.00}_{-0.00}$ & $1200.00^{+0.00}_{-0.00}$ & $100.00^{+0.00}_{-0.00}$ \\[3pt]
0780561601 & 3.82 &	$6.14^{+0.00}_{-0.00}$ & $5.00^{+2.41}_{-0.00}$ & $2.4^{+0.00}_{-0.00}$ & $2.3^{+0.00}_{-0.00}$ & $1.00^{+0.00}_{-0.00}$	& $3.00^{+0.00}_{-0.00}$ & $1000.00^{+0.00}_{-211.35}$ & $20.00^{+17.65}_{-2.68}$ \\[3pt]
0780561701 & 0.26 &	$6.28^{+0.13}_{-0.04}$ & $6.00^{+0.00}_{-0.00}$ & $2.2^{+0.00}_{-0.00}$ & $1.9^{+0.00}_{-0.00}$ & $3.00^{+0.00}_{-0.00}$	& $1.00^{+0.00}_{-0.00}$ & $1200.00^{+0.00}_{-0.00}$ & $100.00^{+0.00}_{-0.00}$ \\[3pt]
0792180101 & 0.54 &	$6.38^{+0.07}_{-0.07}$ & $17.00^{+0.00}_{-0.00}$ & $2.4^{+0.00}_{-0.00}$ & $1.7^{+0.00}_{-0.00}$ & $3.00^{+0.00}_{-0.00}$	& $3.00^{+0.00}_{-0.00}$ & $500.00^{+0.00}_{-212.52}$ & $20.00^{+0.00}_{-0.00}$ \\[3pt]
0792180201 & 0.52 &	$6.22^{+0.05}_{-0.05}$ & $20.00^{+0.00}_{-0.00}$ & $2.4^{+0.00}_{-0.00}$ & $1.9^{+0.00}_{-0.00}$ & $2.00^{+0.00}_{-0.00}$	& $2.00^{+0.00}_{-0.00}$ & $400.00^{+0.00}_{-200.21}$ & $30.00^{+0.00}_{-0.00}$ \\[3pt]
0792180301 & 0.33 &	$6.50^{+0.03}_{-0.02}$ & $16.00^{+0.00}_{-6.61}$ & $2.7^{+0.00}_{-0.59}$ & $2.1^{+0.00}_{-0.00}$ & $1.00^{+0.00}_{-0.00}$	& $3.00^{+0.00}_{-1.17}$ & $300.00^{+310.62}_{-26.44}$ & $20.00^{+4.50}_{-5.01}$ \\[3pt]
0792180401 & 1.26 &	$6.36^{+0.04}_{-0.05}$ & $20.00^{+0.00}_{-8.38}$ & $2.9^{+0.00}_{-0.00}$ & $2.4^{+0.00}_{-0.00}$ & $3.00^{+0.00}_{-0.00}$	& $3.00^{+0.00}_{-0.00}$ & $1000.00^{+0.00}_{-767.15}$ & $20.00^{+9.84}_{-5.43}$ \\ [3pt]
0792180501 & 0.75 &	$6.33^{+0.07}_{-0.07}$ & $16.00^{+0.00}_{-0.00}$ & $2.8^{+0.00}_{-0.00}$ & $2.3^{+0.00}_{-0.00}$ & $1.00^{+0.00}_{-0.00}$	& $3.00^{+0.00}_{-0.00}$ & $500.00^{+0.00}_{-0.00}$ & $20.00^{+16.25}_{-0.00}$ \\ [3pt]
0792180601 & 0.62 &	$6.27^{+0.06}_{-0.12}$ & $3.00^{+0.00}_{-0.00}$ & $2.2^{+0.00}_{-0.00}$ & $1.9^{+0.00}_{-0.00}$ & $2.00^{+0.00}_{-0.00}$	& $1.00^{+0.00}_{-0.00}$ & $600.00^{+0.00}_{-339.56}$ & $90.00^{+0.00}_{-0.00}$ \\ [3pt]
\hline 
\end{tabular}
\end{table}


% 1H0707-495 FITS


\begin{figure}
\centering
% TRIM={A,B,C,D} = {Left, Bottom, Right, Top}
% eg:  [trim={0.0cm 0 1.5cm 0.8cm},clip,scale=0.6]{images/1H0707_tm_comb.pdf}
    \includegraphics[trim={0.5cm 0.5cm 3.2cm 0.8cm},clip,scale=0.33]{images/1H0707-495_tm_comb.pdf}
    \put(-70,140){Combined}
    \includegraphics[trim={0.5cm 0.5cm 3.2cm 0.8cm},clip,scale=0.33]{images/1H0707-495_tm_hiflux.pdf}
    \put(-60,140){Hi-flux}\\
    \includegraphics[trim={0.5cm 0.5cm 3.2cm 0.8cm},clip,scale=0.33]{images/1H0707-495_tm_hicts.pdf}
    \put(-90,140){Hi-cts (\textgreater 20 cts s$^{-1}$)}
    \includegraphics[trim={0.5cm 0.5cm 3.2cm 0.8cm},clip,scale=0.33]{images/1H0707-495_tm_medflux.pdf}
    \put(-60,140){Med-flux}\\
    \includegraphics[trim={0.5cm 0.5cm 3.2cm 0.8cm},clip,scale=0.33]{images/1H0707-495_tm_loflux.pdf}
    \put(-60,140){Lo-flux}
    %\put(-190,50)\rotatebox{90}{{\small{Time lag (s)}}}
    \put(-140,-8){\small{Fequency (Hz)}}
    \includegraphics[trim={0.5cm 0.5cm 3.2cm 0.8cm},clip,scale=0.33]{images/1H0707-495_tm_locts.pdf}
    \put(-90,140){Lo-cts (\textless 20 cts s$^{-1}$)}
    \put(-140,-8){\small{Fequency (Hz)}}
    \vspace{0.5cm}
\caption[ECM fits for 1H 0707-495]{Time lag versus frequency plots for the 1H 0707-495 grouped data. The observed time lags on the $x$-axis are shown in blue and the ECM model fit is shown in red. The reverberation spectrum is shown by the grey wavy line (note this closely follows a zero lag in the medium flux state). All 6 groups are shown beginning with the combined data as labelled \emph{(top left)}, through to the low-counts group \emph{(bottom right)}.}
\label{fig:1h_TM_ECM_plots}
\end{figure} 

\twocolumn 

% IARS 13224-3809 FITS
\onecolumn

\begin{figure}
\centering
% TRIM={A,B,C,D} = {Left, Bottom, Right, Top}
% eg:  [trim={0.0cm 0 1.5cm 0.8cm},clip,scale=0.6]{images/1H0707_tm_comb.pdf}
    \includegraphics[trim={0.5cm 0.75cm 3.2cm 0.8cm},clip,scale=0.33]{images/IRAS13224-3809_tm_comb.pdf}
    \put(-70,140){Combined}
    \includegraphics[trim={0.5cm 0.75cm 3.2cm 0.8cm},clip,scale=0.33]{images/IRAS13224-3809_tm_hiflux.pdf}
    \put(-60,140){Hi-flux}\\
    \includegraphics[trim={0.5cm 0.75cm 3.2cm 0.8cm},clip,scale=0.33]{images/IRAS13224-3809_tm_hicts.pdf}
    \put(-90,140){Hi-cts (\textgreater 20 cts s$^{-1}$)}
    \includegraphics[trim={0.5cm 0.75cm 3.2cm 0.8cm},clip,scale=0.33]{images/IRAS13224-3809_tm_medflux.pdf}
    \put(-60,140){Med-flux}\\
    \includegraphics[trim={0.5cm 0.75cm 3.2cm 0.8cm},clip,scale=0.33]{images/IRAS13224-3809_tm_loflux.pdf}
    \put(-60,140){Lo-flux}
    %\put(-190,50)\rotatebox{90}{{\small{Time lag (s)}}}
    \put(-140,-8){\small{Fequency (Hz)}}
    \includegraphics[trim={0.5cm 0.75cm 3.2cm 0.8cm},clip,scale=0.33]{images/IRAS13224-3809_tm_locts.pdf}
    \put(-90,140){Lo-cts (\textless 20 cts s$^{-1}$)}
    \put(-140,-8){\small{Fequency (Hz)}}
    \vspace{0.5cm}
\caption[ECM fits for IRAS 13224-3809]{Time lag versus frequency plots for the IRAS 13224-3809 grouped data. The observed time lags on the $x$-axis are shown in blue and the ECM model fit is shown in red. The reverberation spectrum is shown by the grey wavy line. All 6 groups are shown beginning with the combined data as labelled \emph{(top left)}, through to the low-counts group \emph{(bottom right)}.}
\label{fig:IRAS_TM_ECM_plots}
\end{figure} 

\twocolumn 



\begin{figure}
    \centering
    % TRIM={A,B,C,D} = {Left, Bottom, Right, Top}
    \includegraphics[trim={0.5cm 0cm 0.5cm 1.0cm},clip,scale=0.44]{images/1H_ECM_h2_lag.pdf}
    \includegraphics[trim={0.5cm 0cm 0.5cm 1.0cm},clip,scale=0.44]{images/IRAS_ECM_h2_lag.pdf}
    \caption{Extended corona model upper source height  results for 1H 0707-495 \emph{(top panel)} and IRAS 13224-3809 \emph{(bottom panel)} plotted against the time lag. The red line indicates the best linear fit for both AGN.}
% /home/steff075/phd_ecm/results-spectral/1H_ECM_h2_lag.py and IRAS_ECM_h2_lag.py 
    \label{fig:ecm_h2_lag}
\end{figure} 


\begin{table}
\centering
\caption[Extended Corona Model parameters]{The extended corona model parameter assumptions for 1H 0707-495.} 
\label{ecm-initial-pars}
\begin{tabular}{ccc}
\\ \hline 
{Parameter} & {Fixed/Free}  & {Range} \\ \hline
$log M$ & Free & $5.5 - 8$  \\[1pt] 
$i$ & Fixed & $53^\circ$ \\[1pt]
$a$ & Fixed & $0.998$ \\[1pt]
$h_1$ & Fixed & $2r_g$ \\[1pt]
$h_2$ & Free & $3 - 20r_g$    \\[1pt]
$\Gamma_1$ & Free & $1.5 - 3.3$   \\[1pt]
$\Gamma_2$ & Free & $1.4 - 3.2$   \\[1pt]
$Fe$ & Fixed &  $1$ (solar abundance) \\[1pt]
$\xi$ & Free &  $0 - 3$ ergs cm s$^{-1}$ \\[1pt]
$p$ & Fixed &  $0$ (constant) \\[1pt]
$b$ & Free &  $1 - 3$\\[1pt]
$q_2$ & Fixed & $0.5$ \\[1pt]
$t_\text{max}$ & Free &  $100 - 800t_g$  \\[1pt]
$t_\text{shift}$ & Free &  $10 - 120t_g$ \\[1pt] 
\hline
\end{tabular}
\end{table}


\begin{figure}
% PATH = /data/typhon1/reverb/1H0707-495/isis_emcee/1H0707-comb-fit-emcee.sl
% TRIM={A,B,C,D} = {Left, Bottom, Right, Top}
    \centering
    \includegraphics[trim={0.5cm 0 3.2cm 1.8cm},clip,scale=0.33]{images/1H0707_comb_fmax_logmass.pdf}\\
    \includegraphics[trim={0.5cm 0 3.2cm 1.8cm},clip,scale=0.33]{images/1H0707_comb_fmax_chain_hist2d.pdf}
%    \put(-155,220){\small{lag\_freq(1).log\_mass}}
%    \put(-155,-10){\small{lag\_freq(1).log\_mass}}    
    \caption{1H 0707-495 posterior density \emph{(top panel)} for the combined observations showing the mean mass $\mu$ = 6.22 (solid blue line) and $\sigma$ = 0.01 (black dashed lines) and the contour plot of the model mass and normalisation \emph{(bottom panel)}. }
    \label{fig:1h_mass_density_emcee}
\end{figure} 


\begin{figure}
% PATH = /data/typhon1/reverb/1H0707-495/isis_emcee/1H0707-comb-fit-emcee.sl
% TRIM={A,B,C,D} = {Left, Bottom, Right, Top}
\centering
\includegraphics[trim={0.5cm 0.8cm 3.2cm 1.8cm},clip,scale=0.32]{images/IRAS_comb_tm_bc_logmass.pdf} \put(-145,-10){\small{lag\_freq(1).log\_mass}} \\
\includegraphics[trim={0.5cm 0.8cm 3.2cm 2.0cm},clip,scale=0.32]{images/IRAS_comb_tm_bc_chain_hist2d.pdf}
\put(-145,-10){\small{lag\_freq(1).log\_mass}} \\
% \put(-135,-10){\small{Frequency (Hz)}}     
\caption{IRAS 13224-3809 posterior density \emph{(top panel)} for the combined observations showing the mean mass $\mu$ = 6.34 (solid blue line) and $\sigma$ = 0.01 (black dashed lines) and the contour plot of the model mass and normalisation \emph{(bottom panel)}.}
\label{fig:IRAS_mass_density_emcee}
\end{figure} 

